Comparing interpretation methods in mental state decoding analyses with deep learning models

Deep learning (DL) models find increasing application in mental state decoding, where researchers seek to understand the mapping between mental states (e.g., perceiving fear or joy) and brain activity by identifying those brain regions (and networks) whose activity allows to accurately identify (i.e., decode) these states. Once a DL model has been trained to accurately decode a set of mental states, neuroimaging researchers often make use of interpretation methods from explainable artificial intelligence research to understand the model's learned mappings between mental states and brain activity. Here, we compare the explanation performance of prominent interpretation methods in a mental state decoding analysis of three functional Magnetic Resonance Imaging (fMRI) datasets. Our findings demonstrate a gradient between two key characteristics of an explanation in mental state decoding, namely, its biological plausibility and faithfulness: interpretation methods with high explanation faithfulness, which capture the model's decision process well, generally provide explanations that are biologically less plausible than the explanations of interpretation methods with less explanation faithfulness. Based on this finding, we provide specific recommendations for the application of interpretation methods in mental state decoding.

==> sections/methods/glm-analysis.tex <==
This analysis
included an indicator vector for each mental state of the dataset, and a set 
of nuisance regressors, namely, an indicator vector for each of the ten 
model training runs as well as an indicator vector for each experimental run 
in the data. We also included a nuisance regressor describing the 
sum of attribution values for each trial-level map, as the total sum of
attribution values can vary highly between decoding decisions (e.g., due to varying 
decoding certainty of the model). By use of this subject-level regression model, 
we then contrasted each mental state of a dataset against all other mental states of the
dataset, resulting in one subject-level attribution map for each mental state. 

In a second step of this analysis, we performed a
group-level GLM analysis of the individual subject-level attribution maps by the
use of the standard two-stage procedure for random-effects group-level analyses as 
proposed by~\citep{holmes_generalisability_1998}. This analysis
included an indicator vector for each contrast type (i.e., mental state) as well as a nuisance indicator 
vector for each subject. The resulting group-level attribution maps thus correspond to a 
paired, two-sample t-test over the subject-level attribution maps. Note that we applied spatial smoothing with a 5mm FWHM Gaussian kernel to all subject-level attribution maps for the group-level GLM analysis.

We also repeated this GLM analysis procedure for the trial-level BOLD maps of each
dataset (without the nuisance regressors for model training runs and
attribution sums), to identify the set of brain 
regions whose activity we would expect to be associated with each mental state 
in a standard analysis of the BOLD data.
